Harnessing the Latent Diffusion Model for Training-Free Image Style Transfer

Diffusion models have recently shown the ability to generate high-quality images. However, controlling its generation process still poses challenges. The image style transfer task is one of those challenges that transfers the visual attributes of a style image to another content image. Typical obstacle of this task is the requirement of additional training of a pre-trained model. We propose a training-free style transfer algorithm, Style Tracking Reverse Diffusion Process (STRDP) for a pretrained Latent Diffusion Model (LDM). Our algorithm employs Adaptive Instance Normalization (AdaIN) function in a distinct manner during the reverse diffusion process of an LDM while tracking the encoding history of the style image. This algorithm enables style transfer in the latent space of LDM for reduced computational cost, and provides compatibility for various LDM models. Through a series of experiments and a user study, we show that our method can quickly transfer the style of an image without additional training. The speed, compatibility, and training-free aspect of our algorithm facilitates agile experiments with combinations of styles and LDMs for extensive application.

==> Makefile <==
# Root directory of your LaTeX project
PROJECT_ROOT = .

# Find all PDF files recursively in the project directory
PDFS = $(shell find $(PROJECT_ROOT) -type f -name "*.pdf")

# Temporary directory for storing compressed files
TEMP_DIR = temp_compressed

# Log file
LOG_FILE = compression_log.txt

# Compression target
compress: $(PDFS)
	@mkdir -p $(TEMP_DIR)
	@echo "Starting PDF compression process at $$(date)" | tee $(LOG_FILE)
	@echo "Found $$(echo $(PDFS) | wc -w) PDF files to compress" | tee -a $(LOG_FILE)
	@echo "" | tee -a $(LOG_FILE)
	@$(foreach pdf,$(PDFS),\
		echo "Processing: $(pdf)" | tee -a $(LOG_FILE); \
		original_size=$$(du -h "$(pdf)" | cut -f1); \
		mkdir -p $(TEMP_DIR)/$(dir $(pdf)); \
		gs -sDEVICE=pdfwrite -dCompatibilityLevel=1.4 -dPDFSETTINGS=/prepress \
		-dColorImageResolution=300 -dGrayImageResolution=300 \
		-dMonoImageResolution=300 -dNOPAUSE -dQUIET -dBATCH \
		-sOutputFile=$(TEMP_DIR)/$(pdf) $(pdf); \
		compressed_size=$$(du -h "$(TEMP_DIR)/$(pdf)" | cut -f1); \
		mv $(TEMP_DIR)/$(pdf) $(pdf); \
		echo "  Original size: $$original_size" | tee -a $(LOG_FILE); \
		echo "  Compressed size: $$compressed_size" | tee -a $(LOG_FILE); \
		echo "  Compressed file replaced original" | tee -a $(LOG_FILE); \
		echo "" | tee -a $(LOG_FILE);)
	@rm -rf $(TEMP_DIR)
	@echo "Compression process completed at $$(date)" | tee -a $(LOG_FILE)
	@echo "Log saved to $(LOG_FILE)"

# Clean target (optional, removes all PDF files - use with caution!)
clean:
	@echo "Cleaning up PDF files..."
	@rm -f $(PDFS)
	@echo "All PDF files have been removed."

.PHONY: compress clean


==> rating/13_2_raw.tex <==
\begin{tabular}{l|r|rrr}
\toprule
 & Gatys $et al.$ & Huang $et al.$ & StyTr$^2$ & QuantArt & InST & DiffuseIT & Ours \\
\midrule
Overall Quality & 2.666667 & 2.000000 & 2.333333 & 1.333333 & 2.333333 & 1.666667 & 2.333333 \\
Color Preservation & 1.666667 & 2.000000 & 1.333333 & 2.666667 & 2.333333 & 3.000000 & 3.000000 \\
Shape Preservation & 3.666667 & 3.000000 & 2.666667 & 3.333333 & 2.000000 & 3.666667 & 2.333333 \\
Texture Transfer & 3.333333 & 2.000000 & 2.333333 & 1.000000 & 2.333333 & 1.333333 & 2.000000 \\
\bottomrule
\end{tabular}


==> rating/14_3_raw.tex <==
\begin{tabular}{l|r|rrr}
\toprule
 & Gatys $et al.$ & Huang $et al.$ & StyTr$^2$ & QuantArt & InST & DiffuseIT & Ours \\
\midrule
Overall Quality & 2.000000 & 3.666667 & 3.333333 & 3.333333 & 1.666667 & 3.000000 & 2.666667 \\
Color Preservation & 1.666667 & 2.666667 & 2.666667 & 2.000000 & 2.333333 & 2.000000 & 3.000000 \\
Shape Preservation & 3.000000 & 3.666667 & 3.666667 & 3.666667 & 1.000000 & 3.333333 & 3.666667 \\
Texture Transfer & 3.333333 & 2.000000 & 3.333333 & 2.666667 & 2.000000 & 1.666667 & 3.333333 \\
\bottomrule
\end{tabular}


==> rating/15_0_raw.tex <==
\begin{tabular}{l|r|rrr}
\toprule
 & Gatys $et al.$ & Huang $et al.$ & StyTr$^2$ & QuantArt & InST & DiffuseIT & Ours \\
\midrule
Overall Quality & 3.333333 & 3.000000 & 3.666667 & 3.666667 & 4.000000 & 2.666667 & 3.333333 \\
Color Preservation & 2.666667 & 2.666667 & 2.666667 & 1.333333 & 2.666667 & 1.666667 & 2.666667 \\
Shape Preservation & 3.333333 & 4.333333 & 5.000000 & 3.666667 & 3.666667 & 2.666667 & 3.666667 \\
Texture Transfer & 4.000000 & 3.333333 & 4.666667 & 1.666667 & 2.666667 & 1.666667 & 1.666667 \\
\bottomrule
\end{tabular}


==> rating/19_1_raw.tex <==
\begin{tabular}{l|r|rrr}
\toprule
 & Gatys $et al.$ & Huang $et al.$ & StyTr$^2$ & QuantArt & InST & DiffuseIT & Ours \\
\midrule
Overall Quality & 3.666667 & 3.000000 & 4.000000 & 3.333333 & 2.333333 & 2.333333 & 3.000000 \\
Color Preservation & 2.666667 & 2.666667 & 2.666667 & 3.333333 & 2.000000 & 1.666667 & 4.000000 \\
Shape Preservation & 5.000000 & 4.333333 & 4.666667 & 4.000000 & 2.666667 & 2.666667 & 2.333333 \\
Texture Transfer & 3.666667 & 3.000000 & 5.000000 & 2.333333 & 3.000000 & 3.666667 & 3.333333 \\
\bottomrule
\end{tabular}


==> rating/1_0_raw.tex <==
\begin{tabular}{l|r|rrr}
\toprule
 & Gatys $et al.$ & Huang $et al.$ & StyTr$^2$ & QuantArt & InST & DiffuseIT & Ours \\
\midrule
Overall Quality & 1.666667 & 1.666667 & 3.000000 & 3.666667 & 1.666667 & 2.666667 & 2.333333 \\
Color Preservation & 2.333333 & 2.000000 & 1.000000 & 3.333333 & 2.333333 & 1.000000 & 3.000000 \\
Shape Preservation & 4.000000 & 3.333333 & 3.666667 & 4.000000 & 1.666667 & 3.666667 & 3.333333 \\
Texture Transfer & 4.000000 & 2.333333 & 3.333333 & 1.666667 & 1.333333 & 3.333333 & 2.666667 \\
\bottomrule
\end{tabular}


==> rating/21_2_raw.tex <==
\begin{tabular}{l|r|rrr}
\toprule
 & Gatys $et al.$ & Huang $et al.$ & StyTr$^2$ & QuantArt & InST & DiffuseIT & Ours \\
\midrule
Overall Quality & 4.000000 & 3.666667 & 4.000000 & 4.666667 & 1.666667 & 4.333333 & 3.333333 \\
Color Preservation & 4.333333 & 3.666667 & 3.333333 & 4.666667 & 2.000000 & 4.000000 & 4.000000 \\
Shape Preservation & 4.666667 & 4.666667 & 4.333333 & 4.333333 & 2.000000 & 4.333333 & 3.666667 \\
Texture Transfer & 5.000000 & 5.000000 & 2.666667 & 3.333333 & 1.666667 & 3.000000 & 2.000000 \\
\bottomrule
\end{tabular}


==> rating/35_3_raw.tex <==
\begin{tabular}{l|r|rrr}
\toprule
 & Gatys $et al.$ & Huang $et al.$ & StyTr$^2$ & QuantArt & InST & DiffuseIT & Ours \\
\midrule
Overall Quality & 3.000000 & 1.333333 & 3.666667 & 4.000000 & 2.333333 & 1.666667 & 3.666667 \\
Color Preservation & 3.000000 & 1.333333 & 1.333333 & 3.000000 & 2.333333 & 1.000000 & 3.333333 \\
Shape Preservation & 3.666667 & 2.666667 & 4.666667 & 4.000000 & 1.666667 & 2.000000 & 3.000000 \\
Texture Transfer & 3.333333 & 2.333333 & 3.666667 & 2.666667 & 1.666667 & 1.666667 & 2.333333 \\
\bottomrule
\end{tabular}


==> rating/6_1_raw.tex <==
\begin{tabular}{l|r|rrr}
\toprule
 & Gatys $et al.$ & Huang $et al.$ & StyTr$^2$ & QuantArt & InST & DiffuseIT & Ours \\
\midrule
Overall Quality & 3.000000 & 3.666667 & 3.666667 & 5.000000 & 2.000000 & 1.666667 & 2.000000 \\
Color Preservation & 3.333333 & 3.333333 & 3.333333 & 3.666667 & 2.333333 & 3.000000 & 4.666667 \\
Shape Preservation & 2.666667 & 3.666667 & 4.333333 & 3.666667 & 1.666667 & 2.666667 & 4.333333 \\
Texture Transfer & 4.666667 & 3.333333 & 4.333333 & 3.666667 & 2.666667 & 2.333333 & 4.000000 \\
\bottomrule
\end{tabular}


==> rating/_13704,__wikiart_,_7080,__places365_large_val___0.tex <==
\begin{tabular}{lrrrr}
 & Overall Quality & Content Color Preservation & Shape Preservation & Texture Transfer \\
\hline
AdaIN & 3.00 & 2.67 & 4.33 & 3.33 \\
DiffuseIT & 2.67 & 1.67 & 2.67 & 1.67 \\
Gatys $et \ al.$ & 3.33 & 2.67 & 3.33 & 4.00 \\
InST & 4.00 & 2.67 & 3.67 & 2.67 \\
\textbf{Ours} & 3.33 & 2.67 & 3.67 & 1.67 \\
QuantArt & 3.67 & 1.33 & 3.67 & 1.67 \\
StyTr$^2$ & 3.67 & 2.67 & 5.00 & 4.67 \\
\end{tabular}

==> rating/_24021,__wikiart_,_29226,__imagenet_val___1.tex <==
\begin{tabular}{lrrrr}
\textbf{} & Overall Quality & Content Color Preservation & Shape Preservation & Texture Transfer \\
\hline
AdaIN & 3.00 & 2.67 & 4.33 & 3.00 \\
DiffuseIT & 2.33 & 1.67 & 2.67 & 3.67 \\
Gatys $et \ al.$ & 3.67 & 2.67 & 5.00 & 3.67 \\
InST & 2.33 & 2.00 & 2.67 & 3.00 \\
\textbf{Ours} & 3.00 & 4.00 & 2.33 & 3.33 \\
QuantArt & 3.33 & 3.33 & 4.00 & 2.33 \\
StyTr$^2$ & 4.00 & 2.67 & 4.67 & 5.00 \\
\hline
\end{tabular}

==> rating/_26300,__wikiart_,_34827,__places365_large_val___2.tex <==
\begin{tabular}{lrrrr}
\hline
Overall Quality & Content Color Preservation & Shape Preservation & Texture Transfer \\
\hline
AdaIN & 3.67 & 3.67 & 4.67 & 5.00 \\
DiffuseIT & 4.33 & 4.00 & 4.33 & 3.00 \\
Gatys $et \ al.$ & 4.00 & 4.33 & 4.67 & 5.00 \\
InST & 1.67 & 2.00 & 2.00 & 1.67 \\
\textbf{Ours} & 3.33 & 4.00 & 3.67 & 2.00 \\
QuantArt & 4.67 & 4.67 & 4.33 & 3.33 \\
StyTr$^2$ & 4.00 & 3.33 & 4.33 & 2.67 \\
\hline
\end{tabular}

==> rating/_68511,__wikiart_,_33553,__imagenet_val___3.tex <==
\begin{tabular}{lrrrr}
 & Overall Quality & Content Color Preservation & Shape Preservation & Texture Transfer \\
\hline
AdaIN & 1.33 & 1.33 & 2.67 & 2.33 \\
DiffuseIT & 1.67 & 1.00 & 2.00 & 1.67 \\
Gatys $et \ al.$ & 3.00 & 3.00 & 3.67 & 3.33 \\
InST & 2.33 & 2.33 & 1.67 & 1.67 \\
\textbf{Ours} & \textbf{3.67} & \textbf{3.33} & \textbf{3.00} & \textbf{2.33} \\
QuantArt & 4.00 & 3.00 & 4.00 & 2.67 \\
StyTr$^2$ & 3.67 & 1.33 & 4.67 & 3.67 \\
\end{tabular}

==> tables/metrics.tex <==
\begin{tabular}{lrrrrrr}
 & Style Loss \textdownarrow & Content Loss \textdownarrow & LPIPS \textdownarrow & PSNR \textuparrow & SSIM \textuparrow & CLIP \textuparrow \\
Huang $et\ al.$ & {\cellcolor[HTML]{482071}} \color[HTML]{F1F1F1} 0.016 & {\cellcolor[HTML]{1FA187}} \color[HTML]{F1F1F1} 14.8 & {\cellcolor[HTML]{FDE725}} \color[HTML]{000000} 0.70 & {\cellcolor[HTML]{481769}} \color[HTML]{F1F1F1} 13.00 & {\cellcolor[HTML]{471063}} \color[HTML]{F1F1F1} 0.29 & {\cellcolor[HTML]{38598C}} \color[HTML]{F1F1F1} 0.62 \\
Gatys $et\ al.$ & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} 0.012 & {\cellcolor[HTML]{2FB47C}} \color[HTML]{F1F1F1} 16.0 & {\cellcolor[HTML]{EAE51A}} \color[HTML]{000000} 0.69 & {\cellcolor[HTML]{30698E}} \color[HTML]{F1F1F1} 16.05 & {\cellcolor[HTML]{2F6C8E}} \color[HTML]{F1F1F1} 0.40 & {\cellcolor[HTML]{38598C}} \color[HTML]{F1F1F1} 0.62 \\
StyTr$^2$ & {\cellcolor[HTML]{471164}} \color[HTML]{F1F1F1} 0.014 & {\cellcolor[HTML]{25838E}} \color[HTML]{F1F1F1} 12.5 & {\cellcolor[HTML]{7AD151}} \color[HTML]{000000} 0.63 & {\cellcolor[HTML]{414487}} \color[HTML]{F1F1F1} 14.53 & {\cellcolor[HTML]{54C568}} \color[HTML]{000000} 0.54 & {\cellcolor[HTML]{20A386}} \color[HTML]{F1F1F1} 0.75 \\
QuantArt & {\cellcolor[HTML]{40BD72}} \color[HTML]{F1F1F1} 0.045 & {\cellcolor[HTML]{2E6D8E}} \color[HTML]{F1F1F1} 11.0 & {\cellcolor[HTML]{37B878}} \color[HTML]{F1F1F1} 0.58 & {\cellcolor[HTML]{3B528B}} \color[HTML]{F1F1F1} 15.08 & {\cellcolor[HTML]{3A548C}} \color[HTML]{F1F1F1} 0.37 & {\cellcolor[HTML]{40BD72}} \color[HTML]{F1F1F1} 0.80 \\
InST & {\cellcolor[HTML]{FDE725}} \color[HTML]{000000} 0.060 & {\cellcolor[HTML]{AADC32}} \color[HTML]{000000} 19.9 & {\cellcolor[HTML]{73D056}} \color[HTML]{000000} 0.62 & {\cellcolor[HTML]{414287}} \color[HTML]{F1F1F1} 14.50 & {\cellcolor[HTML]{482878}} \color[HTML]{F1F1F1} 0.31 & {\cellcolor[HTML]{481A6C}} \color[HTML]{F1F1F1} 0.54 \\
DiffuseIT & {\cellcolor[HTML]{DFE318}} \color[HTML]{000000} 0.057 & {\cellcolor[HTML]{25848E}} \color[HTML]{F1F1F1} 12.6 & {\cellcolor[HTML]{E2E418}} \color[HTML]{000000} 0.69 & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} 12.34 & {\cellcolor[HTML]{3C508B}} \color[HTML]{F1F1F1} 0.36 & {\cellcolor[HTML]{25858E}} \color[HTML]{F1F1F1} 0.70 \\
Ours(S=0.1) & {\cellcolor[HTML]{ADDC30}} \color[HTML]{000000} 0.054 & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} 4.9 & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} 0.33 & {\cellcolor[HTML]{FDE725}} \color[HTML]{000000} 23.28 & {\cellcolor[HTML]{FDE725}} \color[HTML]{000000} 0.63 & {\cellcolor[HTML]{FDE725}} \color[HTML]{000000} 0.93 \\
Ours(S=0.3) & {\cellcolor[HTML]{40BD72}} \color[HTML]{F1F1F1} 0.045 & {\cellcolor[HTML]{2B748E}} \color[HTML]{F1F1F1} 11.5 & {\cellcolor[HTML]{297A8E}} \color[HTML]{F1F1F1} 0.48 & {\cellcolor[HTML]{5EC962}} \color[HTML]{000000} 20.56 & {\cellcolor[HTML]{3ABA76}} \color[HTML]{F1F1F1} 0.52 & {\cellcolor[HTML]{27AD81}} \color[HTML]{F1F1F1} 0.77 \\
Ours(S=0.5) & {\cellcolor[HTML]{1F9F88}} \color[HTML]{F1F1F1} 0.038 & {\cellcolor[HTML]{3FBC73}} \color[HTML]{F1F1F1} 16.8 & {\cellcolor[HTML]{32B67A}} \color[HTML]{F1F1F1} 0.57 & {\cellcolor[HTML]{1F998A}} \color[HTML]{F1F1F1} 18.20 & {\cellcolor[HTML]{297B8E}} \color[HTML]{F1F1F1} 0.42 & {\cellcolor[HTML]{3A538B}} \color[HTML]{F1F1F1} 0.61 \\
Ours(S=0.7) & {\cellcolor[HTML]{21918C}} \color[HTML]{F1F1F1} 0.036 & {\cellcolor[HTML]{A0DA39}} \color[HTML]{000000} 19.6 & {\cellcolor[HTML]{86D549}} \color[HTML]{000000} 0.63 & {\cellcolor[HTML]{2D718E}} \color[HTML]{F1F1F1} 16.39 & {\cellcolor[HTML]{39568C}} \color[HTML]{F1F1F1} 0.37 & {\cellcolor[HTML]{48186A}} \color[HTML]{F1F1F1} 0.53 \\
Ours(S=0.9) & {\cellcolor[HTML]{23898E}} \color[HTML]{F1F1F1} 0.034 & {\cellcolor[HTML]{FDE725}} \color[HTML]{000000} 22.1 & {\cellcolor[HTML]{FDE725}} \color[HTML]{000000} 0.70 & {\cellcolor[HTML]{482979}} \color[HTML]{F1F1F1} 13.61 & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} 0.28 & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} 0.51 \\
\end{tabular}


==> tables/table_metrics.tex <==
\begin{tabular}{lrrllll}
 & Style Loss \textdownarrow & Content Loss \textdownarrow & LPIPS \textdownarrow & PSNR \textuparrow & SSIM \textuparrow & CLIP \textuparrow \\
Huang $et\ al.$ & {\cellcolor[HTML]{482071}} \color[HTML]{F1F1F1} 0.016 & {\cellcolor[HTML]{1FA187}} \color[HTML]{F1F1F1} 14.8 & {\cellcolor[HTML]{FDE725}} \color[HTML]{000000} 0.70 & {\cellcolor[HTML]{481769}} \color[HTML]{F1F1F1} 13.00 & {\cellcolor[HTML]{471063}} \color[HTML]{F1F1F1} 0.29 & {\cellcolor[HTML]{38598C}} \color[HTML]{F1F1F1} 0.62 \\
Gatys $et\ al.$ & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} 0.012 & {\cellcolor[HTML]{2FB47C}} \color[HTML]{F1F1F1} 16.0 & {\cellcolor[HTML]{EAE51A}} \color[HTML]{000000} 0.69 & {\cellcolor[HTML]{30698E}} \color[HTML]{F1F1F1} 16.05 & {\cellcolor[HTML]{2F6C8E}} \color[HTML]{F1F1F1} 0.40 & {\cellcolor[HTML]{38598C}} \color[HTML]{F1F1F1} 0.62 \\
StyTr$^2$ & {\cellcolor[HTML]{471164}} \color[HTML]{F1F1F1} 0.014 & {\cellcolor[HTML]{25838E}} \color[HTML]{F1F1F1} 12.5 & {\cellcolor[HTML]{7AD151}} \color[HTML]{000000} 0.63 & {\cellcolor[HTML]{414487}} \color[HTML]{F1F1F1} 14.53 & {\cellcolor[HTML]{54C568}} \color[HTML]{000000} 0.54 & {\cellcolor[HTML]{20A386}} \color[HTML]{F1F1F1} 0.75 \\
QuantArt & {\cellcolor[HTML]{40BD72}} \color[HTML]{F1F1F1} 0.045 & {\cellcolor[HTML]{2E6D8E}} \color[HTML]{F1F1F1} 11.0 & {\cellcolor[HTML]{37B878}} \color[HTML]{F1F1F1} 0.58 & {\cellcolor[HTML]{3B528B}} \color[HTML]{F1F1F1} 15.08 & {\cellcolor[HTML]{3A548C}} \color[HTML]{F1F1F1} 0.37 & {\cellcolor[HTML]{40BD72}} \color[HTML]{F1F1F1} 0.80 \\
InST & {\cellcolor[HTML]{FDE725}} \color[HTML]{000000} 0.060 & {\cellcolor[HTML]{AADC32}} \color[HTML]{000000} 19.9 & {\cellcolor[HTML]{73D056}} \color[HTML]{000000} 0.62 & {\cellcolor[HTML]{414287}} \color[HTML]{F1F1F1} 14.50 & {\cellcolor[HTML]{482878}} \color[HTML]{F1F1F1} 0.31 & {\cellcolor[HTML]{481A6C}} \color[HTML]{F1F1F1} 0.54 \\
DiffuseIT & {\cellcolor[HTML]{DFE318}} \color[HTML]{000000} 0.057 & {\cellcolor[HTML]{25848E}} \color[HTML]{F1F1F1} 12.6 & {\cellcolor[HTML]{E2E418}} \color[HTML]{000000} 0.69 & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} 12.34 & {\cellcolor[HTML]{3C508B}} \color[HTML]{F1F1F1} 0.36 & {\cellcolor[HTML]{25858E}} \color[HTML]{F1F1F1} 0.70 \\
Ours(S=0.1) & {\cellcolor[HTML]{ADDC30}} \color[HTML]{000000} 0.054 & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} 4.9 & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} 0.33 & {\cellcolor[HTML]{FDE725}} \color[HTML]{000000} 23.28 & {\cellcolor[HTML]{FDE725}} \color[HTML]{000000} 0.63 & {\cellcolor[HTML]{FDE725}} \color[HTML]{000000} 0.93 \\
Ours(S=0.3) & {\cellcolor[HTML]{40BD72}} \color[HTML]{F1F1F1} 0.045 & {\cellcolor[HTML]{2B748E}} \color[HTML]{F1F1F1} 11.5 & {\cellcolor[HTML]{297A8E}} \color[HTML]{F1F1F1} 0.48 & {\cellcolor[HTML]{5EC962}} \color[HTML]{000000} 20.56 & {\cellcolor[HTML]{3ABA76}} \color[HTML]{F1F1F1} 0.52 & {\cellcolor[HTML]{27AD81}} \color[HTML]{F1F1F1} 0.77 \\
Ours(S=0.5) & {\cellcolor[HTML]{1F9F88}} \color[HTML]{F1F1F1} 0.038 & {\cellcolor[HTML]{3FBC73}} \color[HTML]{F1F1F1} 16.8 & {\cellcolor[HTML]{32B67A}} \color[HTML]{F1F1F1} 0.57 & {\cellcolor[HTML]{1F998A}} \color[HTML]{F1F1F1} 18.20 & {\cellcolor[HTML]{297B8E}} \color[HTML]{F1F1F1} 0.42 & {\cellcolor[HTML]{3A538B}} \color[HTML]{F1F1F1} 0.61 \\
Ours(S=0.7) & {\cellcolor[HTML]{21918C}} \color[HTML]{F1F1F1} 0.036 & {\cellcolor[HTML]{A0DA39}} \color[HTML]{000000} 19.6 & {\cellcolor[HTML]{86D549}} \color[HTML]{000000} 0.63 & {\cellcolor[HTML]{2D718E}} \color[HTML]{F1F1F1} 16.39 & {\cellcolor[HTML]{39568C}} \color[HTML]{F1F1F1} 0.37 & {\cellcolor[HTML]{48186A}} \color[HTML]{F1F1F1} 0.53 \\
Ours(S=0.9) & {\cellcolor[HTML]{23898E}} \color[HTML]{F1F1F1} 0.034 & {\cellcolor[HTML]{FDE725}} \color[HTML]{000000} 22.1 & {\cellcolor[HTML]{FDE725}} \color[HTML]{000000} 0.70 & {\cellcolor[HTML]{482979}} \color[HTML]{F1F1F1} 13.61 & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} 0.28 & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} 0.51 \\
\end{tabular}


==> tables/table_metrics_refined.tex <==
\begin{tabular}{l|c|c|c|c|c|c}
\hline
 & Style Loss\textdownarrow & Content Loss\textdownarrow & PSNR\textdownarrow & LPIPS\textuparrow & SSIM\textuparrow & CLIP\textuparrow \\
\hline
Huang $et\ al.$ & {\cellcolor[HTML]{482071}} \color[HTML]{F1F1F1} 0.016 & {\cellcolor[HTML]{1FA187}} \color[HTML]{F1F1F1} 14.8 & {\cellcolor[HTML]{E5E419}} \color[HTML]{000000} 0.70 & {\cellcolor[HTML]{38598C}} \color[HTML]{F1F1F1} 0.62 & {\cellcolor[HTML]{481769}} \color[HTML]{F1F1F1} 13.0 & {\cellcolor[HTML]{471063}} \color[HTML]{F1F1F1} 0.29 \\
Gatys $et\ al.$ & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} 0.012 & {\cellcolor[HTML]{2FB47C}} \color[HTML]{F1F1F1} 16.0 & {\cellcolor[HTML]{CAE11F}} \color[HTML]{000000} 0.68 & {\cellcolor[HTML]{38598C}} \color[HTML]{F1F1F1} 0.62 & {\cellcolor[HTML]{30698E}} \color[HTML]{F1F1F1} 16.0 & {\cellcolor[HTML]{2F6C8E}} \color[HTML]{F1F1F1} 0.40 \\
StyTr$^2$ & {\cellcolor[HTML]{471164}} \color[HTML]{F1F1F1} 0.014 & {\cellcolor[HTML]{25838E}} \color[HTML]{F1F1F1} 12.5 & {\cellcolor[HTML]{75D054}} \color[HTML]{000000} 0.61 & {\cellcolor[HTML]{20A386}} \color[HTML]{F1F1F1} 0.75 & {\cellcolor[HTML]{414487}} \color[HTML]{F1F1F1} 14.5 & {\cellcolor[HTML]{54C568}} \color[HTML]{000000} 0.54 \\
QuantArt & {\cellcolor[HTML]{40BD72}} \color[HTML]{F1F1F1} 0.045 & {\cellcolor[HTML]{2E6D8E}} \color[HTML]{F1F1F1} 11.0 & {\cellcolor[HTML]{20A486}} \color[HTML]{F1F1F1} 0.50 & {\cellcolor[HTML]{40BD72}} \color[HTML]{F1F1F1} 0.80 & {\cellcolor[HTML]{3B528B}} \color[HTML]{F1F1F1} 15.1 & {\cellcolor[HTML]{3A548C}} \color[HTML]{F1F1F1} 0.37 \\
InST & {\cellcolor[HTML]{FDE725}} \color[HTML]{000000} 0.060 & {\cellcolor[HTML]{AADC32}} \color[HTML]{000000} 19.9 & {\cellcolor[HTML]{A8DB34}} \color[HTML]{000000} 0.65 & {\cellcolor[HTML]{481A6C}} \color[HTML]{F1F1F1} 0.54 & {\cellcolor[HTML]{414287}} \color[HTML]{F1F1F1} 14.5 & {\cellcolor[HTML]{482878}} \color[HTML]{F1F1F1} 0.31 \\
DiffuseIT & {\cellcolor[HTML]{DFE318}} \color[HTML]{000000} 0.057 & {\cellcolor[HTML]{25848E}} \color[HTML]{F1F1F1} 12.6 & {\cellcolor[HTML]{C2DF23}} \color[HTML]{000000} 0.67 & {\cellcolor[HTML]{25858E}} \color[HTML]{F1F1F1} 0.70 & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} 12.3 & {\cellcolor[HTML]{3C508B}} \color[HTML]{F1F1F1} 0.36 \\
\hline
Ours(S=0.1) & {\cellcolor[HTML]{ADDC30}} \color[HTML]{000000} 0.054 & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} 4.9 & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} 0.19 & {\cellcolor[HTML]{FDE725}} \color[HTML]{000000} 0.93 & {\cellcolor[HTML]{FDE725}} \color[HTML]{000000} 23.3 & {\cellcolor[HTML]{FDE725}} \color[HTML]{000000} 0.63 \\
Ours(S=0.3) & {\cellcolor[HTML]{40BD72}} \color[HTML]{F1F1F1} 0.045 & {\cellcolor[HTML]{2B748E}} \color[HTML]{F1F1F1} 11.5 & {\cellcolor[HTML]{2D718E}} \color[HTML]{F1F1F1} 0.39 & {\cellcolor[HTML]{27AD81}} \color[HTML]{F1F1F1} 0.77 & {\cellcolor[HTML]{5EC962}} \color[HTML]{000000} 20.6 & {\cellcolor[HTML]{3ABA76}} \color[HTML]{F1F1F1} 0.52 \\
Ours(S=0.5) & {\cellcolor[HTML]{1F9F88}} \color[HTML]{F1F1F1} 0.038 & {\cellcolor[HTML]{3FBC73}} \color[HTML]{F1F1F1} 16.8 & {\cellcolor[HTML]{38B977}} \color[HTML]{F1F1F1} 0.55 & {\cellcolor[HTML]{3A538B}} \color[HTML]{F1F1F1} 0.61 & {\cellcolor[HTML]{1F998A}} \color[HTML]{F1F1F1} 18.2 & {\cellcolor[HTML]{297B8E}} \color[HTML]{F1F1F1} 0.42 \\
Ours(S=0.7) & {\cellcolor[HTML]{21918C}} \color[HTML]{F1F1F1} 0.036 & {\cellcolor[HTML]{A0DA39}} \color[HTML]{000000} 19.6 & {\cellcolor[HTML]{A5DB36}} \color[HTML]{000000} 0.65 & {\cellcolor[HTML]{48186A}} \color[HTML]{F1F1F1} 0.53 & {\cellcolor[HTML]{2D718E}} \color[HTML]{F1F1F1} 16.4 & {\cellcolor[HTML]{39568C}} \color[HTML]{F1F1F1} 0.37 \\
Ours(S=0.9) & {\cellcolor[HTML]{23898E}} \color[HTML]{F1F1F1} 0.034 & {\cellcolor[HTML]{FDE725}} \color[HTML]{000000} 22.1 & {\cellcolor[HTML]{FDE725}} \color[HTML]{000000} 0.72 & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} 0.51 & {\cellcolor[HTML]{482979}} \color[HTML]{F1F1F1} 13.6 & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} 0.28 \\
\hline
\end{tabular}


==> tables/table_metrics_v2.tex <==
\begin{tabular}{l|c|c|c|c|c|c}
\hline
 & Style Loss \textdownarrow & Content Loss \textdownarrow & LPIPS \textdownarrow & PSNR \textuparrow & SSIM \textuparrow & CLIP \textuparrow \\
 \hline
Huang $et\ al.$ & {\cellcolor[HTML]{482071}} \color[HTML]{F1F1F1} 0.016 & {\cellcolor[HTML]{1FA187}} \color[HTML]{F1F1F1} 14.8 & {\cellcolor[HTML]{FDE725}} \color[HTML]{000000} 0.70 & {\cellcolor[HTML]{481769}} \color[HTML]{F1F1F1} 13.00 & {\cellcolor[HTML]{471063}} \color[HTML]{F1F1F1} 0.3 & {\cellcolor[HTML]{38598C}} \color[HTML]{F1F1F1} 0.62 \\
Gatys $et\ al.$ & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} 0.012 & {\cellcolor[HTML]{2FB47C}} \color[HTML]{F1F1F1} 16.0 & {\cellcolor[HTML]{EAE51A}} \color[HTML]{000000} 0.69 & {\cellcolor[HTML]{30698E}} \color[HTML]{F1F1F1} 16.05 & {\cellcolor[HTML]{2F6C8E}} \color[HTML]{F1F1F1} 0.4 & {\cellcolor[HTML]{38598C}} \color[HTML]{F1F1F1} 0.62 \\
StyTr$^2$ & {\cellcolor[HTML]{471164}} \color[HTML]{F1F1F1} 0.014 & {\cellcolor[HTML]{25838E}} \color[HTML]{F1F1F1} 12.5 & {\cellcolor[HTML]{7AD151}} \color[HTML]{000000} 0.63 & {\cellcolor[HTML]{414487}} \color[HTML]{F1F1F1} 14.53 & {\cellcolor[HTML]{54C568}} \color[HTML]{000000} 0.5 & {\cellcolor[HTML]{20A386}} \color[HTML]{F1F1F1} 0.75 \\
QuantArt & {\cellcolor[HTML]{40BD72}} \color[HTML]{F1F1F1} 0.045 & {\cellcolor[HTML]{2E6D8E}} \color[HTML]{F1F1F1} 11.0 & {\cellcolor[HTML]{37B878}} \color[HTML]{F1F1F1} 0.58 & {\cellcolor[HTML]{3B528B}} \color[HTML]{F1F1F1} 15.08 & {\cellcolor[HTML]{3A548C}} \color[HTML]{F1F1F1} 0.4 & {\cellcolor[HTML]{40BD72}} \color[HTML]{F1F1F1} 0.80 \\
InST & {\cellcolor[HTML]{FDE725}} \color[HTML]{000000} 0.060 & {\cellcolor[HTML]{AADC32}} \color[HTML]{000000} 19.9 & {\cellcolor[HTML]{73D056}} \color[HTML]{000000} 0.62 & {\cellcolor[HTML]{414287}} \color[HTML]{F1F1F1} 14.50 & {\cellcolor[HTML]{482878}} \color[HTML]{F1F1F1} 0.3 & {\cellcolor[HTML]{481A6C}} \color[HTML]{F1F1F1} 0.54 \\
DiffuseIT & {\cellcolor[HTML]{DFE318}} \color[HTML]{000000} 0.057 & {\cellcolor[HTML]{25848E}} \color[HTML]{F1F1F1} 12.6 & {\cellcolor[HTML]{E2E418}} \color[HTML]{000000} 0.69 & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} 12.34 & {\cellcolor[HTML]{3C508B}} \color[HTML]{F1F1F1} 0.4 & {\cellcolor[HTML]{25858E}} \color[HTML]{F1F1F1} 0.70 \\
\hline
Ours(S=0.1) & {\cellcolor[HTML]{ADDC30}} \color[HTML]{000000} 0.054 & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} 4.9 & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} 0.33 & {\cellcolor[HTML]{FDE725}} \color[HTML]{000000} 23.28 & {\cellcolor[HTML]{FDE725}} \color[HTML]{000000} 0.6 & {\cellcolor[HTML]{FDE725}} \color[HTML]{000000} 0.93 \\
Ours(S=0.3) & {\cellcolor[HTML]{40BD72}} \color[HTML]{F1F1F1} 0.045 & {\cellcolor[HTML]{2B748E}} \color[HTML]{F1F1F1} 11.5 & {\cellcolor[HTML]{297A8E}} \color[HTML]{F1F1F1} 0.48 & {\cellcolor[HTML]{5EC962}} \color[HTML]{000000} 20.56 & {\cellcolor[HTML]{3ABA76}} \color[HTML]{F1F1F1} 0.5 & {\cellcolor[HTML]{27AD81}} \color[HTML]{F1F1F1} 0.77 \\
Ours(S=0.5) & {\cellcolor[HTML]{1F9F88}} \color[HTML]{F1F1F1} 0.038 & {\cellcolor[HTML]{3FBC73}} \color[HTML]{F1F1F1} 16.8 & {\cellcolor[HTML]{32B67A}} \color[HTML]{F1F1F1} 0.57 & {\cellcolor[HTML]{1F998A}} \color[HTML]{F1F1F1} 18.20 & {\cellcolor[HTML]{297B8E}} \color[HTML]{F1F1F1} 0.4 & {\cellcolor[HTML]{3A538B}} \color[HTML]{F1F1F1} 0.61 \\
Ours(S=0.7) & {\cellcolor[HTML]{21918C}} \color[HTML]{F1F1F1} 0.036 & {\cellcolor[HTML]{A0DA39}} \color[HTML]{000000} 19.6 & {\cellcolor[HTML]{86D549}} \color[HTML]{000000} 0.63 & {\cellcolor[HTML]{2D718E}} \color[HTML]{F1F1F1} 16.39 & {\cellcolor[HTML]{39568C}} \color[HTML]{F1F1F1} 0.4 & {\cellcolor[HTML]{48186A}} \color[HTML]{F1F1F1} 0.53 \\
Ours(S=0.9) & {\cellcolor[HTML]{23898E}} \color[HTML]{F1F1F1} 0.034 & {\cellcolor[HTML]{FDE725}} \color[HTML]{000000} 22.1 & {\cellcolor[HTML]{FDE725}} \color[HTML]{000000} 0.70 & {\cellcolor[HTML]{482979}} \color[HTML]{F1F1F1} 13.61 & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} 0.3 & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} 0.51 \\
\hline
\end{tabular}


==> texs/rating_0.tex <==
\begin{table*}[ht]
\centering
\begin{tabular*}{\textwidth}{p{0.5\textwidth} p{0.4\textwidth}}
\hline
\textbf{Inputs and Results} & \textbf{Average User Rating} \\ 
\hline
\includegraphics[width=\linewidth]{inouts/0_0.pdf} & \includegraphics[width=\linewidth]{rating/0_0.pdf} \\ 
\hline
\includegraphics[width=\linewidth]{inouts/0_1.pdf} & \includegraphics[width=\linewidth]{rating/0_1.pdf} \\ 
\hline
\includegraphics[width=\linewidth]{inouts/0_2.pdf} & \includegraphics[width=\linewidth]{rating/0_2.pdf} \\ 
\hline
\includegraphics[width=\linewidth]{inouts/0_3.pdf} & \includegraphics[width=\linewidth]{rating/0_3.pdf} \\ 
\hline
\end{tabular*}
\caption{Examples of style transfer results and user ratings.} 
\label{tab:rating0}
\end{table*}
